Unsupervised Commonsense Question Answering with Self-Talk

Natural language understanding involves reading between the lines with implicit background knowledge. Current systems either rely on pre-trained language models as the sole implicit source of world knowledge, or resort to external knowledge bases (KBs) to incorporate additional relevant knowledge. We propose an unsupervised framework based on self-talk as a novel alternative to multiple-choice commonsense tasks. Inspired by inquiry-based discovery learning (Bruner, 1961), our approach inquires language models with a number of information seeking questions such as "$\textit{what is the definition of ...}$" to discover additional background knowledge. Empirical results demonstrate that the self-talk procedure substantially improves the performance of zero-shot language model baselines on four out of six commonsense benchmarks, and competes with models that obtain knowledge from external KBs. While our approach improves performance on several benchmarks, the self-talk induced knowledge even when leading to correct answers is not always seen as useful by human judges, raising interesting questions about the inner-workings of pre-trained language models for commonsense reasoning.

==> archive/clarification_examples.tex <==
\setlength\tabcolsep{1.8pt}
\begin{tabular}{>{\raggedright\arraybackslash}p{2cm} >{\raggedright\arraybackslash}p{1.5cm} >{\raggedright\arraybackslash}p{6cm} >{\raggedright\arraybackslash}p{4cm} >{\raggedright\arraybackslash}p{5cm} >{\raggedright\arraybackslash}p{5cm}}
\toprule
\textbf{Task} & \textbf{Knowledge Source} & \textbf{Context + \textit{Question}} & \textbf{Correct Answer} & \textbf{Clarification Question} & \textbf{Clarification} \\ 
\midrule
\multirow{2}{*}{\copa} & \comet{} & The player caught the ball. \textit{What was the cause for it?} & Her teammate threw it to her. & Before that, what did the player need? & Before, the player needed to go to the ball field.\\
\hhline{~-----}
& ConceptNet & The boy skipped dinner. \textit{What was the cause for it?} & He ate a big lunch. & What is the relationship between `dinner' and `lunch'? & Lunch is the opposite of dinner.\\
\midrule
\multirow{2}{*}{\commonsenseqa} & ConceptNet & \textit{Working on the elaborate task was taxing, it require extreme what?} & concentration & What is the relationship between `working' and `concentration'? & In order for working to happen, concentration needs to happen.\\
\hhline{~-----}
& DistilGPT2 & \textit{What do professors primarily do?} & teach courses & What is the main function of a professor's teaching career,? & The main function of a professor's teaching career, is to teach students how they can improve their knowledge.\\
\midrule
\multirow{2}{*}{\mctaco} & GPT2-XL & Growing up on a farm near St. Paul, L. Mark Bailey didn't dream of becoming a judge. \textit{How many years did it take for Mark to become a judge?} & 7 years & What happened first? & The first thing that happened was he went to law school and became an attorney.\\
\hhline{~-----}
& GPT & After several years of private practice from 1982-90, he became the judge of Decatur County Court for a year. \textit{When did he get a law degree?} & 1981 & What happened first? & The first thing that happened was that his wife, linda, had passed away.\\
\midrule
\multirow{6}{*}{\socialiqa} & \comet{} & Bailey saved money because they wanted to buy something good. \textit{How would you describe Bailey?} & Bailey is seen as good with money. & How would you describe Bailey? & Bailey is seen as hardworking. \\
\hhline{~-----}
& ConceptNet & Jan had been on vacation in Hawaii for a week. Last night, she finally returned home. \textit{What will Jan want to do next?} & As a result, Jan wanted to return to work. & What is the relationship between `vacation' and `work'?	& Vacation is the opposite of work. \\
\hhline{~-----}
& DistilGPT2 & Robin proposed another solution after the first one was not successful. \textit{What does Robin need to do before this?} & Before, Robin needed to come up with other solutions. & What does Robin need to do before this? & Before doing that, Robin first had to do some research on how he could make it.\\
\hhline{~-----}
& GPT2 & Skylar always arrives 15 minutes early for class, takes extensive notes, and studies hard before tests. \textit{How would you describe Skylar?} & Skylar is seen as a dedicated student. & How would you describe Skylar? & Skylar is a very good student who does well in the classroom.\\
\hhline{~-----}
& GPT2-M & Carson was at a friends house and they decided to play video games. \textit{What does Carson need to do before this?} & Before, Carson needed to know about their friends house. & What does Carson need to do before this? & Before doing that, Carson first had to get his mother's permission before playing the game.\\
\hhline{~-----}
& GPT2-L & Taylor gave a raise and a promotion to Kendall. \textit{How would you describe Taylor?} & Taylor is seen as as someone who appreciates what Kendall does. & How would you describe Taylor? & Taylor is a good guy, but he's also an idiot.\\
\midrule
\multirow{4}{*}{\piqa} & \comet{} & To cut circles out of dough without a cookie cutter. & Use a glass by turning it upside down and using the rim. & What does you want as a result? & As a result, you wants to get the dough out of the oven.\\
\hhline{~-----}
& ConceptNet & How can I slice up a banana? & Use a knife, on a cutting board, and slice the banana into quarter sized slices. & What is the relationship between `slice' and `knife'? & Slice is a specific way of doing cut. Knife is used for cut.\\
\hhline{~-----}
& GPT2-XL & What pan to use for frying eggs? & Nonstick pans are perfect for frying eggs. & What is the definition of a `pan'? & The definition of a `pan' is : A metal or ceramic vessel used in cooking.\\
\hhline{~-----}
& XLNet-base & Sharpen a pencil. & Use a knife. & What are the properties of a you sharpen a pencil,? & The properties of a you sharpen a pencil, are that it will not break or be dulled.\\
\midrule
\winogrande & \comet{} & Joel complained to Ian about the condition of the house. \_ preferred a messy space. & Ian & What does Joel want as a result? & As a result, Joel wants to get rid of the clutter. \\
\hhline{~-----}
& GPT2 & The hotel had a terrible gym but a nice restaurant; the \_ was something management attended to. & restaurant & What is the definition of `restaurant'? & `restaurant' is defined as an establishment that serves food, drinks and services.\\
\hhline{~-----}
& GPT2-M & Mark wanted to lose some weight by starting a diet and workout routine. He focused mainly on the \_ because he was lazy. & diet & What is the definition of `workout routine'? & `workout routine' is defined as any kind of exercise that involves doing physical activity.\\
\hhline{~-----}
& GPT2-XL & The parakeet flew to Hunter but flew past Samuel because \_ had some bird seed in their hand. & Hunter & What does it mean to be a `bird'? & Be a `bird' means the same thing as it does for us humans.\\
\hhline{~-----}
& GPT & Matt wanted to change either the plain bathroom or the colorful bedroom, but the \_ was already colorful. & bedroom &	What is the definition of `bedroom'? & `bedroom' is defined as a room with a bed and nightstand in it.\\
\hhline{~-----}
& XLNet-base & My employer offers a bonus of either a phone or a television, but unfortunately the \_ is just way too large to be useful. & phone & What is the definition of `phone'? & `phone' is defined as device that connects a person directly into the world.\\
\bottomrule
\end{tabular}






==> archive/task_examples.tex <==
\setlength\tabcolsep{1.8pt}
\begin{tabular}{l l l}
\toprule
\textbf{Dataset} & \textbf{Context + \textit{Question}} & \textbf{Choices} \\ 
\midrule
\copa & The man broke his toe. \textit{What was the cause of this?} & 1) He got a hole in his sock. \textbf{2) He dropped a hammer on his foot.} \\
\midrule
\commonsenseqashort & \textit{Where on a river can you hold a cup upright to catch water on a sunny day?} & \textbf{1) waterfall} 2) bridge 3) valley 4) pebble 5) mountain \\ 
\midrule
\mctaco & [...] becoming a judge. \textit{How many years did it take [...] to become a judge?} & 1) 63 years 2) 7 weeks \textbf{3) 7 years} 4) 7 seconds 5) 7 hours \\
\midrule
\multirow{2}{*}{\socialiqa} & [...] Robin played a hero in the struggle to the death with the angry villain. & 1) sorry for the villain  \textbf{2) hopeful that Robin will succeed} \\
&  \textit{How would others feel as a result?} & 3) like Robin should lose the fight \\ 
\midrule
\multirow{2}{*}{\piqa} & \textit{To separate egg whites from the yolk using a water bottle, you should} & \textbf{1) [...] Release, which creates suction and lifts the yolk.} \\
& & 2) [...] Keep pushing, which creates suction and lifts the yolk. \\
\midrule
\multirow{2}{*}{\winogrande} & Katrina had the financial means to afford a new car while Monica did not,  & \textbf{1) Katrina} \\
& since \_ had a high paying job. & 2) Monica \\
\bottomrule
\end{tabular}





